Transient Non-Stationarity and Generalisation in Deep Reinforcement Learning

Non-stationarity can arise in Reinforcement Learning (RL) even in stationary environments. For example, most RL algorithms collect new data throughout training, using a non-stationary behaviour policy. Due to the transience of this non-stationarity, it is often not explicitly addressed in deep RL and a single neural network is continually updated. However, we find evidence that neural networks exhibit a memory effect where these transient non-stationarities can permanently impact the latent representation and adversely affect generalisation performance. Consequently, to improve generalisation of deep RL agents, we propose Iterated Relearning (ITER). ITER augments standard RL training by repeated knowledge transfer of the current policy into a freshly initialised network, which thereby experiences less non-stationarity during training. Experimentally, we show that ITER improves performance on the challenging generalisation benchmarks ProcGen and Multiroom.

==> core/8_impact.tex <==
\section*{Broader Impact}
We hope our findings are of use both to improve our understanding of how networks learn and
to improve generalisation in \gls{RL} in particular.
Generalisation is important for many applications of \gls{RL} since 
the number of situations a deployed agent can encounter can 
vastly exceed the number of (even approximate) states that can be feasibly observed during training.
One obvious example is autonomous driving, where weather, lighting, traffic participants, and other
objects can always create new, unique situations.
As a result, deploying learned \gls{RL} agents outside of simulations  often 
suffers from a large {\em generalisation gap}, i.e., lower performance in deployment than during
training.
If \gls{RL} agents control important systems, poor generalisation can lead to 
dangerous errors.
Conversely, if they generalise well \gls{RL} agents can be deployed safely and 
effectively in more contexts.

In deep \gls{RL} we rely on neural networks to generalise.
Unfortunately, much about how or why neural networks generalise is still 
unknown.
In this work, we both advance our understanding of the generalisation problem 
in deep \gls{RL}, and propose an algorithmic approach to improve generalisation.
This line of work may help us realise the potential benefits of 
\gls{RL} agents, which may be able to perform useful tasks or aid human 
decision makers in solving difficult problems.
Of course, there are many other challenges in building safe and useful \gls{RL} 
agents, such as specifying reward functions that align well with intended 
behaviours.
Furthermore, improved generalisation in a simulated environment should not give 
over-confidence that agents will generalise well to dramatically different 
states (such as from simulation to the real world, or from one real world 
setting to another).
Lastly, without a thorough theoretical understanding of how neural networks learn to generalise, it
is impossible to know under which constraints improvements due to \gls{ITER} can be guaranteed, if
at all.
We hope that our experiments prove to be helpful for further advances in this direction, but much
works remains to be done.


